A Parabolic Relaxation Model for the Navier-Stokes-Korteweg Equations

The isothermal Navier-Stokes-Korteweg system is a classical diffuse interface model for compressible two-phase flow. However, the numerical solution faces two major challenges: due to a third-order dispersion contribution in the momentum equations, extended numerical stencils are required for the flux calculation. Furthermore, the equation of state given by a Van-der-Waals law, exhibits non-monotone behaviour in the two-phase state space leading to imaginary eigenvalues of the Jacobian of the first-order fluxes. In this work a lower-order parabolic relaxation model is used to approximate solutions of the classical NSK equations. Whereas an additional parabolic evolution equation for the relaxation variable has to be solved, the system involves no differential operator of higher as second order. The use of a modified pressure function guarantees that the first-order fluxes remain hyperbolic. Altogether, the relaxation system is directly accessible for standard compressible flow solvers. We use the higher-order Discontinuous Galerkin spectral element method as realized in the open source code FLEXI. The relaxation model is validated against solutions of the original NSK model for a variety of 1D and 2D test cases. Three-dimensional simulations of head-on droplet collisions for a range of different collision Weber numbers underline the capability of the approach.

==> packages.tex <==
\RequirePackage{etex}
\usepackage{etoolbox}  % insert new e-TEX commands (required for \AfterEndEnvironment)

%-------------------------------------------------------------------------------
% EQUATIONS
%-------------------------------------------------------------------------------
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{breqn}
\usepackage{mathtools}
\usepackage{nicefrac}
\usepackage[llbracket,rrbracket]{stmaryrd}
\usepackage[normalem]{ulem}

%-------------------------------------------------------------------------------
% LANGUAGE
%-------------------------------------------------------------------------------
\usepackage[ngerman,english]{babel} % Sprache 
\usepackage[utf8]{inputenc} % Tippen von Umlauten


%-------------------------------------------------------------------------------
% IMAGES / GRAPHICS
%-------------------------------------------------------------------------------
\usepackage{graphicx}
% color scheme by http://ksrowell.com/blog-visualizing-data/2012/02/02/optimal-colors-for-graphs/
%\definecolor{myblue}{RGB}{57,106,177}
%\definecolor{myorange}{RGB}{218,124,48}
%\definecolor{mygreen}{RGB}{62,150,81}
%\definecolor{myred}{RGB}{204,37,41}
%\definecolor{mygrey}{RGB}{83,81,84}
%\definecolor{mypurple}{RGB}{107,76,154}
%\definecolor{mybrown}{RGB}{146,36,40}
%\definecolor{mybeige}{RGB}{148,139,61}

% color scheme by https://personal.sron.nl/~pault/
\usepackage{xcolor}
% bright scheme
\definecolor{myblue}{RGB}{68,119,170}
\definecolor{mycyan}{RGB}{102,204,238}
\definecolor{mygreen}{RGB}{34,136,51}
\definecolor{myyellow}{RGB}{204,187,68}
\definecolor{myred}{RGB}{238,102,119}
\definecolor{mypurple}{RGB}{170,51,119}
\definecolor{mygrey}{RGB}{187,187,187}

% vibrant scheme
%\definecolor{myblue}{RGB}{0,119,187}
%\definecolor{mycyan}{RGB}{51,187,238}
%\definecolor{mygreen}{RGB}{0,153,136}
%\definecolor{myyellow}{RGB}{238,119,51} % this is acutally orange
%\definecolor{myred}{RGB}{204,51,17}
%\definecolor{mypurple}{RGB}{238,51,119} % this is acutally magenta
%\definecolor{mygrey}{RGB}{187,187,187}

% light scheme
%\definecolor{myblue}{RGB}{119,170,221}
%\definecolor{mycyan}{RGB}{153,221,255}
%\definecolor{mygreen}{RGB}{68,187,153}
%\definecolor{myyellow}{RGB}{238,221,136}
%\definecolor{myred}{RGB}{238,136,102}
%\definecolor{mypurple}{RGB}{255,170,187}
%\definecolor{mygrey}{RGB}{187,187,187}

%-------------------------------------------------------------------------------
% FLOAT CONTROL
%-------------------------------------------------------------------------------
%\usepackage[section]{placeins} # Alle figures,tabellen, etc. innerhalb der section anorden

%-------------------------------------------------------------------------------
% TABULAR
%-------------------------------------------------------------------------------
%\usepackage{supertabular}
%\usepackage{array}
%\usepackage{longtable}
\usepackage{tabularx}
%\renewcommand{\arraystretch}{1.1}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs} % The package enhances the quality of tables

%-------------------------------------------------------------------------------
% CAPTIONS
%-------------------------------------------------------------------------------
\usepackage[format=hang,labelfont=bf]{caption}  % Tabellen/Figure Beschriftung 
\usepackage{subcaption}

% -------------------------------------------------------------------------------
% SI units
% -------------------------------------------------------------------------------
\usepackage{siunitx}
%\sisetup{inter-unit-product =$\cdot$}
\sisetup{exponent-product = \cdot, output-product = \cdot}
%\sisetup{detect-weight, detect-display-math}
%\sisetup{detect-inline-weight=math}
\sisetup{allow-number-unit-breaks}

% Angstrom symbol
\DeclareSIUnit{\angstrom}{\mbox{\normalfont\AA}}
\makeatletter
\DeclareRobustCommand{\AA}{%
  \leavevmode
  \vbox{\ialign{##\cr
    \hidewidth\char'27 \hidewidth\cr
    \noalign{\nointerlineskip\kern-1.4ex}
    A\cr
  }}%
}
\makeatother


%-------------------------------------------------------------------------------
% OTHER USEFUL PACKAGES
%-------------------------------------------------------------------------------
\usepackage{changebar}
\usepackage[mode=image]{standalone}
\usepackage{csquotes}  % Anfuehrungszeichen (wird von glossaries empfohlen)
\usepackage{xspace}    % Leerzeichen oder nicht nach Kommando einfuegen

\usepackage[all]{nowidow} % Witwen und Waisen (Hurenkinder, Schusterjungen) vermeiden

\frenchspacing % No big horizontal spaces between sentences

\usepackage[capitalise]{cleveref}

\newtheorem{thm}{Theorem}[section] 
\newtheorem{remark}[thm]{Remark}


% --------------------------------------------------------------------------------------------------
% Todo plugin
% --------------------------------------------------------------------------------------------------
%% Todo list (can be removed at the end)
\usepackage[colorinlistoftodos,prependcaption]{todonotes}
\presetkeys{todonotes}{inline,color=blue!30,size=\footnotesize}{}

% fix problem when ”\listoftodos” is used in combination with  ”\listoffigures” with the error
% “no room for a new \write”
\usepackage{morewrites} % solution for the error “no room for a new \write”, which occurs when a 
                        % document reserves too many streams to write data to various auxiliary files

%------------------------------------------------------------------------------
% References 
%------------------------------------------------------------------------------
% Die beiden folgen Zeilen sollten eigentlich vor cleveref geladen werden
%\usepackage[
%   backend=biber,
%   maxnames=10,
%   isbn=false,
%   url=false,
%   doi=true,
%   defernumbers=true,
%   giveninits=true,
%   sorting=nyvt,        % nyvt - sort by name, year, volume, title
%%   sorting=none,       % none - sort the entries starting at the beginning       
%   citestyle=numeric-comp, % numeric-comp: compress [1,2,3,4,5] to [1-5]                            
%   noerroretextools=true
%]{biblatex}
%\addbibresource{literature.bib}
%\usepackage{autonum}
% hide more fields                                                                                  
%\AtEveryBibitem{\clearfield{title}}

